Data clustering with edge domination in complex networks

This paper presents a model for a dynamical system where particles dominate edges in a complex network. The proposed dynamical system is then extended to an application on the problem of community detection and data clustering. In the case of the data clustering problem, 6 different techniques were simulated on 10 different datasets in order to compare with the proposed technique. The results show that the proposed algorithm performs well when prior knowledge of the number of clusters is known to the algorithm.

==> Makefile <==
# Copyright © Filipe Neto, Paulo Urio.
#
# Fancy Makefile for LaTeX compiling using latexmk and rubber.
#
# latexmk is used for the actual generation of PDF and cleanup.
# rubber is used for target dependencies scanning and output diagnostics.

# Make options (may be passed by command line, e.g., make BOX=0):
#  BOX    Show bad box messages
#  REF    Show referencing problem messages
#  WARN   Show warning messages
#  ERR    Show error messages
#  CHECK  Show only the most important category of messages.  If there are
#         errors, only errors are displayed; otherwise only warnings if there
#         are, and so on. If CHECK=1, it makes sense to disable every other
#         option.  The disadvantage is that message categories are not colored
#         accordingly.
BOX=1
WARN=1
REF=1
ERR=1
CHECK=0

# Path for LaTeX output files.
# 	BUILD_DIR=.   		Normal build with mixed source and output files.
# 	BUILD_DIR=folder	Separated building; generates all output files in
# 						./folder/, including the PDF.
BUILD_DIR=build

# Main .tex input
TARGET=paper

REL_TARGET=$(shell realpath -q --relative-to=$(BUILD_DIR) $(TARGET))
PDF=$(BUILD_DIR)/$(TARGET).pdf

.PHONY: init all clean cropimages

define colorize
	pretty_$1 := sed -e "s/^\(.*[0-9x]:\)/`tput bold``tput setaf $2`\1`tput sgr0`/"
endef

# Color rules for rubber-info output
$(eval $(call colorize,box,231))
$(eval $(call colorize,warn,226))
$(eval $(call colorize,ref,214))
$(eval $(call colorize,error,196))
$(eval $(call colorize,check,5))

default: $(PDF)

all: cropimages $(PDF)

cropimages:
	@cd images && bash crop.sh --only-tracked-files

# Check whether the variables are valid.
init:
ifeq ($(wildcard $(shell which rubber)),)
	$(error "rubber not found")
endif
ifeq ($(wildcard $(shell which rubber-info)),)
	$(error "rubber-info not found")
endif
ifeq ($(BUILD_DIR),)
	$(error "BUILD_DIR is not set")
endif

scandeps:
ifneq ($(shell rubber-info --deps $(TARGET) | grep ".tex:"),)
	@echo "Scan Dependencies Errors:" | $(pretty_error)
	@rubber-info --deps $(TARGET) | grep ".tex:" | $(pretty_error)
endif

# Generate the main PDF. Target dependencies are scanned with rubber-info.
# Rubber-info won’t get every output message, but it may help us.
$(PDF): init $(BUILD_DIR) scandeps $(shell rubber-info --deps $(TARGET) | grep -v ".tex:")
	@echo "Running latexmk..."
	@-latexmk -pdflatex=lualatex --outdir=$(BUILD_DIR) -pdf -silent $(TARGET)
ifeq ($(BOX),1)
	@cd $(BUILD_DIR) && rubber-info --boxes $(REL_TARGET) | $(pretty_box)
endif
ifeq ($(WARN),1)
	@cd $(BUILD_DIR) && rubber-info --warnings $(REL_TARGET) | $(pretty_warn)
endif
ifeq ($(REF),1)
	@cd $(BUILD_DIR) && rubber-info --refs $(REL_TARGET) | $(pretty_ref)
endif
ifeq ($(ERR),1)
	@cd $(BUILD_DIR) && rubber-info --errors $(REL_TARGET) | $(pretty_error)
endif
ifeq ($(CHECK),1)
	@cd $(BUILD_DIR) && rubber-info --check $(REL_TARGET) | $(pretty_check)
endif

$(BUILD_DIR):
	mkdir -p $(BUILD_DIR)

# Remove files generated by latex and bibtex.
clean: init $(BUILD_DIR)
	@-latexmk --outdir=$(BUILD_DIR) -pdf -silent -c $(TARGET)
	-$(RM) $(PDF) $(PDF:.pdf=.bbl)
ifneq ($(BUILD_DIR),.)
	rmdir $(BUILD_DIR)
endif



==> result_table_real.tex <==
\begin{tabular}{rrrrrrrrrrr}
\toprule
&\TblDatasetName{\pbox{20cm}{Breast\\cancer}}&\TblDatasetName{\pbox{20cm}{Car\\eval.}}&\TblDatasetName{\pbox{20cm}{Credit\\approval}}&\TblDatasetName{\pbox{20cm}{Contr.\\method}}&\TblDatasetName{Glass}&\TblDatasetName{Ion.}&\TblDatasetName{Iris}&\TblDatasetName{Vowel}&\TblDatasetName{Wine}&\TblAvgRankName{\pbox{20cm}{Avg.\\Rank}}\\
\midrule
\TblMethodName{Chameleon}&\TblResultValue{.9557}{.0000}&\TblResultValue{.7993}{.0000}&\TblResultValue{.6349}{.0000}&\TblResultValue{.5539}{.0000}&\TblResultValue{.5373}{.0000}&\TblResultValue{.7094}{.0000}&\TblResultValue{.8867}{.0000}&\TblResultValue{.4778}{.0000}&\TblResultValue{.7022}{.0000}&\TblResultRank{3.7}\\
\TblMethodName{EM}&\TblResultValue{.9193}{.0049}&\TblResultValue{.7103}{.0212}&\TblResultValue{.6294}{.0074}&\TblResultValue{.4425}{.0406}&\TblResultValue{.5081}{.0630}&\TblResultValue{.7308}{.0319}&\TblResultValue{.8766}{.0195}&\TblResultValue{.4694}{.0343}&\TblResultValue{.7134}{.0071}&\TblResultRank{5.9}\\
\TblMethodName{Fuzzy C-means}&\TblResultValue{.9392}{.0031}&\TblResultValue{.7208}{.0192}&\TblResultValue{.6001}{.0026}&\TblResultValue{.5275}{.0295}&\TblResultValue{.5248}{.0170}&\TblResultValue{.7182}{.0095}&\TblResultValue{.8816}{.0584}&\TblResultValue{.4430}{.0296}&\TblResultValue{.7077}{.0061}&\TblResultRank{5.9}\\
\TblMethodName{Opt. \kmeans}&\TblResultValue{.9586}{.0046}&\TblResultValue{.7292}{.0235}&\TblResultValue{.5834}{.0039}&\TblResultValue{.5494}{.0439}&\TblResultValue{.5116}{.0241}&\TblResultValue{.7000}{.0082}&\TblResultValue{.8436}{.0875}&\TblResultValue{.4569}{.0215}&\TblResultValue{.6854}{.0071}&\TblResultRank{6.1}\\
\TblMethodName{Modularity}&\TblResultValue{.9585}{.0000}&\TblResultValue{.7846}{.0000}&\TblResultValue{.5923}{.0000}&\TblResultValue{.5740}{.0000}&\TblResultValue{.5140}{.0000}&\TblResultValue{.7407}{.0000}&\TblResultValue{.9533}{.0000}&\TblResultValue{.4889}{.0000}&\TblResultValue{.7079}{.0000}&\TblResultRank{3.4}\\
\TblMethodName{Particle swarm}&\TblResultValue{.9489}{.0132}&\TblResultValue{.7509}{.0318}&\TblResultValue{.6039}{.0104}&\TblResultValue{.5007}{.0946}&\TblResultValue{.5441}{.1562}&\TblResultValue{.7183}{.0104}&\TblResultValue{.8747}{.0538}&\TblResultValue{.4465}{.0255}&\TblResultValue{.7135}{.0041}&\TblResultRank{4.7}\\
\TblMethodName{Vertice}&\TblResultValue{.9590}{.0074}&\TblResultValue{.7438}{.0143}&\TblResultValue{.6337}{.0039}&\TblResultValue{.5004}{.0450}&\TblResultValue{.5292}{.0656}&\TblResultValue{.7501}{.0298}&\TblResultValue{.8957}{.0227}&\TblResultValue{.4752}{.0145}&\TblResultValue{.7449}{.0162}&\TblResultRank{3.2}\\
\hline
\TblMethodName{\kmeans}&\TblResultValue{.6231}{.0000}&\TblResultValue{.0693}{.0326}&\TblResultValue{.1886}{.1362}&\TblResultValue{.0292}{.0073}&\TblResultValue{.3133}{.0340}&\TblResultValue{.1349}{.0000}&\TblResultValue{.7084}{.0637}&\TblResultValue{.3861}{.0190}&\TblResultValue{.8449}{.0123}&\TblResultRank{9.4}\\
\TblMethodName{DBSCAN+DBCV}&\TblResultValue{.2428}{.0000}&\TblResultValue{.2057}{.0000}&\TblResultValue{.2148}{.0000}&\TblResultValue{.0694}{.0000}&\TblResultValue{.4818}{.0000}&\TblResultValue{.3264}{.0000}&\TblResultValue{.7235}{.0000}&\TblResultValue{.5986}{.0000}&\TblResultValue{.4395}{.0000}&\TblResultRank{8.7}\\
\TblMethodName{Chameleon}&\TblResultValue{.5904}{.0000}&\TblResultValue{.0964}{.0000}&\TblResultValue{.1928}{.0000}&\TblResultValue{.0268}{.0000}&\TblResultValue{.4497}{.0000}&\TblResultValue{.5292}{.0000}&\TblResultValue{.7650}{.0000}&\TblResultValue{.4104}{.0000}&\TblResultValue{.8212}{.0000}&\TblResultRank{8.8}\\
\TblMethodName{\emph{Proposed technique}}&\TblResultValue{.9455}{.0000}&\TblResultValue{.2322}{.0000}&\TblResultValue{.8499}{.0000}&\TblResultValue{.4338}{.0000}&\TblResultValue{.3878}{.0000}&\TblResultValue{.7606}{.0000}&\TblResultValue{.6666}{.0000}&\TblResultValue{.7247}{.0000}&\TblResultValue{.6526}{.0000}&\TblResultRank{6.2}\\
\bottomrule
\end{tabular}
\begin{tabular}{rrrrrrrrrrrr}
\toprule
&\TblDatasetName{\pbox{20cm}{Breast\\cancer}}&\TblDatasetName{\pbox{20cm}{Car\\eval.}}&\TblDatasetName{\pbox{20cm}{Credit\\approval}}&\TblDatasetName{\pbox{20cm}{Contr.\\method}}&\TblDatasetName{Glass}&\TblDatasetName{Ion.}&\TblDatasetName{Iris}&\TblDatasetName{Vowel}&\TblDatasetName{Wine}&\TblDatasetName{Seeds}&\TblAvgRankName{\pbox{20cm}{Avg.\\Rank}}\\
\midrule
\TblMethodName{\kmeans}&\TblResultValue{.7302}{.0000}&\TblResultValue{.0305}{.0215}&\TblResultValue{.2538}{.1803}&\TblResultValue{.0218}{.0066}&\TblResultValue{.1658}{.0279}&\TblResultValue{.1776}{.0000}&\TblResultValue{.6710}{.1050}&\TblResultValue{.1758}{.0166}&\TblResultValue{.8589}{.0122}&\TblResultValue{.7049}{.0000}&\TblResultRank{2.5}\\
\TblMethodName{DBSCAN+DBCV}&\TblResultValue{.2601}{.0000}&\TblResultValue{.0280}{.0000}&\TblResultValue{.0629}{.0000}&\TblResultValue{.0044}{.0000}&\TblResultValue{.2674}{.0000}&\TblResultValue{.5597}{.0000}&\TblResultValue{.5657}{.0000}&\TblResultValue{.0934}{.0000}&\TblResultValue{.3003}{.0000}&\TblResultValue{.3795}{.0000}&\TblResultRank{3.6}\\
\TblMethodName{Chameleon}&\TblResultValue{.7192}{.0000}&\TblResultValue{.1496}{.0000}&\TblResultValue{.1653}{.0000}&\TblResultValue{.0253}{.0000}&\TblResultValue{.2918}{.0000}&\TblResultValue{.6767}{.0000}&\TblResultValue{.6844}{.0000}&\TblResultValue{.1949}{.0000}&\TblResultValue{.8249}{.0000}&\TblResultValue{.7436}{.0000}&\TblResultRank{1.6}\\
\TblMethodName{\emph{Proposed technique}}&\TblResultValue{.7930}{.0000}&\TblResultValue{.0348}{.0000}&\TblResultValue{.4890}{.0000}&\TblResultValue{.0367}{.0000}&\TblResultValue{.2348}{.0000}&\TblResultValue{.2698}{.0000}&\TblResultValue{.5681}{.0000}&\TblResultValue{.1114}{.0000}&\TblResultValue{.5711}{.0000}&\TblResultValue{.5278}{.0000}&\TblResultRank{2.3}\\
\bottomrule
\end{tabular}

